The VLA-COSMOS 3 GHz Large Project: Star formation properties and radio luminosity functions of AGN with moderate-to-high radiative luminosities out to $z\sim6$

We study a sample of 1,604 moderate-to-high radiative luminosity active galactic nuclei (HLAGN) selected at 3 GHz within the VLA-COSMOS 3 GHz Large Project. These were classified by combining multiple AGN diagnostics: X-ray data, mid-infrared data and broad-band spectral energy distribution fitting. We decompose the total radio 1.4 GHz luminosity ($\mathrm{L_{1.4\ GHz,TOT}}$) into the emission originating from star formation and AGN activity by measuring the excess in $\mathrm{L_{1.4\ GHz,TOT}}$ relative to the infrared-radio correlation of star-forming galaxies. To quantify the excess, for each source we calculate the AGN fraction ($\mathrm{f_{AGN}}$), the fractional contribution of AGN activity to $\mathrm{L_{1.4\ GHz,TOT}}$. The majority of the HLAGN, $(68.0\pm1.5)\%$, are dominated by star-forming processes ($f_{AGN}\leq0.5$), while $(32.0\pm1.5)\%$ are dominated by AGN-related radio emission ($0.5<f_{AGN}\leq1$). We use the AGN-related 1.4 GHz emission to derive the 1.4 GHz AGN luminosity functions of HLAGN. By assuming pure density and pure luminosity evolution models we constrain their cosmic evolution out to $z\sim6$, finding $\mathrm{\Phi^* (z) \propto (1+z)^{(2.64\pm0.10)+(-0.61\pm0.04) z}}$ and $\mathrm{L^* (z) \propto (1+z)^{(3.97\pm0.15) + (-0.92\pm0.06)z}}$. These evolutionary laws show that the number and luminosity density of HLAGN increased from higher redshifts ($z\sim6$) up to a maximum in the redshift range $ 1<z<2.5$, followed by a decline towards local values. By scaling the 1.4 GHz AGN luminosity to kinetic luminosity using the standard conversion, we estimate the kinetic luminosity density as a function of redshift. We compare our result to the semi-analytic models of radio mode feedback finding that this feedback could have played an important role in the context of AGN-host coevolution in HLAGN which show evidence of AGN-related radio emission ($f_{AGN}>0$).

==> bibliography.tex <==
@ARTICLE{rigby15,
   author = {{Rigby}, E.~E. and {Argyle}, J. and {Best}, P.~N. and {Rosario}, D. and 
	{R{\"o}ttgering}, H.~J.~A.},
    title = "{Cosmic downsizing of powerful radio galaxies to low radio luminosities}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1507.00341},
 keywords = {galaxies: active, galaxies: high-redshift, galaxies: evolution},
     year = 2015,
    month = sep,
   volume = 581,
      eid = {A96},
    pages = {A96},
      doi = {10.1051/0004-6361/201526475},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...581A..96R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rigby11,
   author = {{Rigby}, E.~E. and {Best}, P.~N. and {Brookes}, M.~H. and {Peacock}, J.~A. and 
	{Dunlop}, J.~S. and {R{\"o}ttgering}, H.~J.~A. and {Wall}, J.~V. and 
	{Ker}, L.},
    title = "{The luminosity-dependent high-redshift turnover in the steep spectrum radio luminosity function: clear evidence for downsizing in the radio-AGN population}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1104.5020},
 keywords = {galaxies: active, galaxies: evolution, galaxies: high-redshift, galaxies: luminosity function, mass function},
     year = 2011,
    month = sep,
   volume = 416,
    pages = {1900-1915},
      doi = {10.1111/j.1365-2966.2011.19167.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.416.1900R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dunlop03,
   author = {{Dunlop}, J.~S. and {McLure}, R.~J. and {Kukula}, M.~J. and 
	{Baum}, S.~A. and {O'Dea}, C.~P. and {Hughes}, D.~H.},
    title = "{Quasars, their host galaxies and their central black holes}",
  journal = {\mnras},
   eprint = {astro-ph/0108397},
 keywords = {black hole physics, galaxies: active, galaxies: photometry, quasars: general, infrared: galaxies},
     year = 2003,
    month = apr,
   volume = 340,
    pages = {1095-1135},
      doi = {10.1046/j.1365-8711.2003.06333.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.340.1095D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{smolcic16,
   author = {{Smolcic}, V.},
    title = "{Radio continuum surveys and galaxy evolution: The AGN view}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1603.05687},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2016,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160305687S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{york00,
   author = {{York}, D.~G. and {Adelman}, J. and {Anderson}, Jr., J.~E. and 
	{Anderson}, S.~F. and {Annis}, J. and {Bahcall}, N.~A. and {Bakken}, J.~A. and 
	{Barkhouser}, R. and {Bastian}, S. and {Berman}, E. and {Boroski}, W.~N. and 
	{Bracker}, S. and {Briegel}, C. and {Briggs}, J.~W. and {Brinkmann}, J. and 
	{Brunner}, R. and {Burles}, S. and {Carey}, L. and {Carr}, M.~A. and 
	{Castander}, F.~J. and {Chen}, B. and {Colestock}, P.~L. and 
	{Connolly}, A.~J. and {Crocker}, J.~H. and {Csabai}, I. and 
	{Czarapata}, P.~C. and {Davis}, J.~E. and {Doi}, M. and {Dombeck}, T. and 
	{Eisenstein}, D. and {Ellman}, N. and {Elms}, B.~R. and {Evans}, M.~L. and 
	{Fan}, X. and {Federwitz}, G.~R. and {Fiscelli}, L. and {Friedman}, S. and 
	{Frieman}, J.~A. and {Fukugita}, M. and {Gillespie}, B. and 
	{Gunn}, J.~E. and {Gurbani}, V.~K. and {de Haas}, E. and {Haldeman}, M. and 
	{Harris}, F.~H. and {Hayes}, J. and {Heckman}, T.~M. and {Hennessy}, G.~S. and 
	{Hindsley}, R.~B. and {Holm}, S. and {Holmgren}, D.~J. and {Huang}, C.-h. and 
	{Hull}, C. and {Husby}, D. and {Ichikawa}, S.-I. and {Ichikawa}, T. and 
	{Ivezi{\'c}}, {\v Z}. and {Kent}, S. and {Kim}, R.~S.~J. and 
	{Kinney}, E. and {Klaene}, M. and {Kleinman}, A.~N. and {Kleinman}, S. and 
	{Knapp}, G.~R. and {Korienek}, J. and {Kron}, R.~G. and {Kunszt}, P.~Z. and 
	{Lamb}, D.~Q. and {Lee}, B. and {Leger}, R.~F. and {Limmongkol}, S. and 
	{Lindenmeyer}, C. and {Long}, D.~C. and {Loomis}, C. and {Loveday}, J. and 
	{Lucinio}, R. and {Lupton}, R.~H. and {MacKinnon}, B. and {Mannery}, E.~J. and 
	{Mantsch}, P.~M. and {Margon}, B. and {McGehee}, P. and {McKay}, T.~A. and 
	{Meiksin}, A. and {Merelli}, A. and {Monet}, D.~G. and {Munn}, J.~A. and 
	{Narayanan}, V.~K. and {Nash}, T. and {Neilsen}, E. and {Neswold}, R. and 
	{Newberg}, H.~J. and {Nichol}, R.~C. and {Nicinski}, T. and 
	{Nonino}, M. and {Okada}, N. and {Okamura}, S. and {Ostriker}, J.~P. and 
	{Owen}, R. and {Pauls}, A.~G. and {Peoples}, J. and {Peterson}, R.~L. and 
	{Petravick}, D. and {Pier}, J.~R. and {Pope}, A. and {Pordes}, R. and 
	{Prosapio}, A. and {Rechenmacher}, R. and {Quinn}, T.~R. and 
	{Richards}, G.~T. and {Richmond}, M.~W. and {Rivetta}, C.~H. and 
	{Rockosi}, C.~M. and {Ruthmansdorfer}, K. and {Sandford}, D. and 
	{Schlegel}, D.~J. and {Schneider}, D.~P. and {Sekiguchi}, M. and 
	{Sergey}, G. and {Shimasaku}, K. and {Siegmund}, W.~A. and {Smee}, S. and 
	{Smith}, J.~A. and {Snedden}, S. and {Stone}, R. and {Stoughton}, C. and 
	{Strauss}, M.~A. and {Stubbs}, C. and {SubbaRao}, M. and {Szalay}, A.~S. and 
	{Szapudi}, I. and {Szokoly}, G.~P. and {Thakar}, A.~R. and {Tremonti}, C. and 
	{Tucker}, D.~L. and {Uomoto}, A. and {Vanden Berk}, D. and {Vogeley}, M.~S. and 
	{Waddell}, P. and {Wang}, S.-i. and {Watanabe}, M. and {Weinberg}, D.~H. and 
	{Yanny}, B. and {Yasuda}, N. and {SDSS Collaboration}},
    title = "{The Sloan Digital Sky Survey: Technical Summary}",
  journal = {\aj},
   eprint = {astro-ph/0006396},
 keywords = {Cosmology: Observations, Instrumentation: Miscellaneous},
     year = 2000,
    month = sep,
   volume = 120,
    pages = {1579-1587},
      doi = {10.1086/301513},
   adsurl = {http://adsabs.harvard.edu/abs/2000AJ....120.1579Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{condon98,
   author = {{Condon}, J.~J. and {Cotton}, W.~D. and {Greisen}, E.~W. and 
	{Yin}, Q.~F. and {Perley}, R.~A. and {Taylor}, G.~B. and {Broderick}, J.~J.
	},
    title = "{The NRAO VLA Sky Survey}",
  journal = {\aj},
 keywords = {CATALOGS, METHODS: DATA ANALYSIS, METHODS: OBSERVATIONAL, RADIO CONTINUUM, SURVEYS},
     year = 1998,
    month = may,
   volume = 115,
    pages = {1693-1716},
      doi = {10.1086/300337},
   adsurl = {http://adsabs.harvard.edu/abs/1998AJ....115.1693C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kapinska14,
   author = {{Kapinska}, A.~D. and {Hardcastle}, M. and {Jackson}, C. and 
	{An}, T. and {Baan}, W. and {Jarvis}, M.},
    title = "{Unravelling lifecycles and physics of radio-loud AGN in the SKA Era}",
  journal = {Advancing Astrophysics with the Square Kilometre Array (AASKA14)},
archivePrefix = "arXiv",
   eprint = {1412.5884},
     year = 2015,
    month = apr,
      eid = {173},
    pages = {173},
   adsurl = {http://adsabs.harvard.edu/abs/2015aska.confE.173K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{capak07,
   author = {{Capak}, P. and {Aussel}, H. and {Ajiki}, M. and {McCracken}, H.~J. and 
	{Mobasher}, B. and {Scoville}, N. and {Shopbell}, P. and {Taniguchi}, Y. and 
	{Thompson}, D. and {Tribiano}, S. and {Sasaki}, S. and {Blain}, A.~W. and 
	{Brusa}, M. and {Carilli}, C. and {Comastri}, A. and {Carollo}, C.~M. and 
	{Cassata}, P. and {Colbert}, J. and {Ellis}, R.~S. and {Elvis}, M. and 
	{Giavalisco}, M. and {Green}, W. and {Guzzo}, L. and {Hasinger}, G. and 
	{Ilbert}, O. and {Impey}, C. and {Jahnke}, K. and {Kartaltepe}, J. and 
	{Kneib}, J.-P. and {Koda}, J. and {Koekemoer}, A. and {Komiyama}, Y. and 
	{Leauthaud}, A. and {Le Fevre}, O. and {Lilly}, S. and {Liu}, C. and 
	{Massey}, R. and {Miyazaki}, S. and {Murayama}, T. and {Nagao}, T. and 
	{Peacock}, J.~A. and {Pickles}, A. and {Porciani}, C. and {Renzini}, A. and 
	{Rhodes}, J. and {Rich}, M. and {Salvato}, M. and {Sanders}, D.~B. and 
	{Scarlata}, C. and {Schiminovich}, D. and {Schinnerer}, E. and 
	{Scodeggio}, M. and {Sheth}, K. and {Shioya}, Y. and {Tasca}, L.~A.~M. and 
	{Taylor}, J.~E. and {Yan}, L. and {Zamorani}, G.},
    title = "{The First Release COSMOS Optical and Near-IR Data and Catalog}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {0704.2430},
 keywords = {Cosmology: Observations, Galaxies: Evolution, Cosmology: Large-Scale Structure of Universe, Surveys},
     year = 2007,
    month = sep,
   volume = 172,
    pages = {99-116},
      doi = {10.1086/519081},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..172...99C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{palomar97,
   author = {{Ho}, L.~C. and {Filippenko}, A.~V. and {Sargent}, W.~L.~W.},
    title = "{A Search for ``Dwarf'' Seyfert Nuclei. III. Spectroscopic Parameters and Properties of the Host Galaxies}",
  journal = {\apjs},
   eprint = {astro-ph/9704107},
 keywords = {GALAXIES: FUNDAMENTAL PARAMETERS, GALAXIES: ACTIVE, GALAXIES: NUCLEI, GALAXIES: SEYFERT, GALAXIES: ISM, Galaxies: Active, Galaxies: Fundamental Parameters, Galaxies: ISM, Galaxies: Nuclei, Galaxies: Seyfert},
     year = 1997,
    month = oct,
   volume = 112,
    pages = {315-390},
      doi = {10.1086/313041},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJS..112..315H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ching17,
   author = {{Ching}, J.~H.~Y. and {Sadler}, E.~M. and {Croom}, S.~M. and 
	{Johnston}, H.~M. and {Pracy}, M.~B. and {Couch}, W.~J. and 
	{Hopkins}, A.~M. and {Jurek}, R.~J. and {Pimbblet}, K.~A.},
    title = "{The Large Area Radio Galaxy Evolution Spectroscopic Survey (LARGESS): survey design, data catalogue and GAMA/WiggleZ spectroscopy}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1609.05578},
 keywords = {catalogues, surveys, galaxies: active, radio continuum: galaxies},
     year = 2017,
    month = jan,
   volume = 464,
    pages = {1306-1332},
      doi = {10.1093/mnras/stw2396},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.464.1306C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hickox09,
   author = {{Hickox}, R.~C. and {Jones}, C. and {Forman}, W.~R. and {Murray}, S.~S. and 
	{Kochanek}, C.~S. and {Eisenstein}, D. and {Jannuzi}, B.~T. and 
	{Dey}, A. and {Brown}, M.~J.~I. and {Stern}, D. and {Eisenhardt}, P.~R. and 
	{Gorjian}, V. and {Brodwin}, M. and {Narayan}, R. and {Cool}, R.~J. and 
	{Kenter}, A. and {Caldwell}, N. and {Anderson}, M.~E.},
    title = "{Host Galaxies, Clustering, Eddington Ratios, and Evolution of Radio, X-Ray, and Infrared-Selected AGNs}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0901.4121},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: active, large-scale structure of universe, quasars: general, radio continuum: galaxies, surveys, X-rays: galaxies},
     year = 2009,
    month = may,
   volume = 696,
    pages = {891-919},
      doi = {10.1088/0004-637X/696/1/891},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...696..891H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{goulding14,
   author = {{Goulding}, A.~D. and {Forman}, W.~R. and {Hickox}, R.~C. and 
	{Jones}, C. and {Murray}, S.~S. and {Paggi}, A. and {Ashby}, M.~L.~N. and 
	{Coil}, A.~L. and {Cooper}, M.~C. and {Huang}, J.-S. and {Kraft}, R. and 
	{Newman}, J.~A. and {Weiner}, B.~J. and {Willner}, S.~P.},
    title = "{Tracing the Evolution of Active Galactic Nuclei Host Galaxies over the Last 9 Gyr of Cosmic Time}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1310.8298},
 keywords = {galaxies: active, galaxies: evolution, galaxies: statistics, infrared: galaxies, radio continuum: galaxies, surveys, X-rays: galaxies},
     year = 2014,
    month = mar,
   volume = 783,
      eid = {40},
    pages = {40},
      doi = {10.1088/0004-637X/783/1/40},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...783...40G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{willott99,
   author = {{Willott}, C.~J. and {Rawlings}, S. and {Blundell}, K.~M. and 
	{Lacy}, M.},
    title = "{The emission line-radio correlation for radio sources using the 7C Redshift Survey}",
  journal = {\mnras},
   eprint = {astro-ph/9905388},
     year = 1999,
    month = nov,
   volume = 309,
    pages = {1017-1033},
      doi = {10.1046/j.1365-8711.1999.02907.x},
   adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.309.1017W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gs16,
   author = {{Godfrey}, L.~E.~H. and {Shabala}, S.~S.},
    title = "{Mutual distance dependence drives the observed jet-power-radio-luminosity scaling relations in radio galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1511.06007},
 keywords = {galaxies: active, galaxies: jets, radio continuum: galaxies},
     year = 2016,
    month = feb,
   volume = 456,
    pages = {1172-1184},
      doi = {10.1093/mnras/stv2712},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.456.1172G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{mh07,
   author = {{Merloni}, A. and {Heinz}, S.},
    title = "{Measuring the kinetic power of active galactic nuclei in the radio mode}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0707.3356},
 keywords = {accretion, accretion discs, black hole physics, galaxies: active, galaxies: evolution, quasars: general},
     year = 2007,
    month = oct,
   volume = 381,
    pages = {589-601},
      doi = {10.1111/j.1365-2966.2007.12253.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.381..589M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mh08,
   author = {{Merloni}, A. and {Heinz}, S.},
    title = "{A synthesis model for AGN evolution: supermassive black holes growth and feedback modes}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0805.2499},
 keywords = {accretion, accretion discs , black hole physics , galaxies: active , galaxies: evolution , quasars: general},
     year = 2008,
    month = aug,
   volume = 388,
    pages = {1011-1030},
      doi = {10.1111/j.1365-2966.2008.13472.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.388.1011M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hardcastle14,
   author = {{Hardcastle}, M.~J. and {Krause}, M.~G.~H.},
    title = "{Numerical modelling of the lobes of radio galaxies in cluster environments - II. Magnetic field configuration and observability}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1406.5300},
 primaryClass = "astro-ph.HE",
 keywords = {hydrodynamics, galaxies: active, galaxies: jets, galaxies: magnetic fields},
     year = 2014,
    month = sep,
   volume = 443,
    pages = {1482-1499},
      doi = {10.1093/mnras/stu1229},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.443.1482H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{kennicutt98,
   author = {{Kennicutt}, Jr., R.~C.},
    title = "{The Global Schmidt Law in Star-forming Galaxies}",
  journal = {\apj},
   eprint = {astro-ph/9712213},
 keywords = {GALAXIES: EVOLUTION, GALAXIES: ISM, GALAXIES: SPIRAL, GALAXIES: STELLAR CONTENT, GALAXIES: STARBURST, STARS: FORMATION, Galaxies: Evolution, Galaxies: ISM, Galaxies: Spiral, Galaxies: Starburst, Galaxies: Stellar Content, Stars: Formation},
     year = 1998,
    month = may,
   volume = 498,
    pages = {541-552},
      doi = {10.1086/305588},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...498..541K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{chabrier,
   author = {{Chabrier}, G.},
    title = "{Galactic Stellar and Substellar Initial Mass Function}",
  journal = {\pasp},
   eprint = {astro-ph/0304382},
 keywords = {Galaxies: Luminosity Function, Mass Function, Invited Reviews},
     year = 2003,
    month = jul,
   volume = 115,
    pages = {763-795},
      doi = {10.1086/376392},
   adsurl = {http://adsabs.harvard.edu/abs/2003PASP..115..763C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{novak17,
   author = {{Novak}, M. and {Smol{\v c}i{\'c}}, V. and {Delhaize}, J. and 
	{Delvecchio}, I. and {Zamorani}, G. and {Baran}, N. and {Bondi}, M. and 
	{Capak}, P. and {Carilli}, C.~L. and {Ciliegi}, P. and {Civano}, F. and 
	{Ilbert}, O. and {Karim}, A. and {Laigle}, C. and {Le F{\`e}vre}, O. and 
	{Marchesi}, S. and {McCracken}, H. and {Miettinen}, O. and {Salvato}, M. and 
	{Sargent}, M. and {Schinnerer}, E. and {Tasca}, L.},
    title = "{The VLA-COSMOS 3 GHz Large Project: Cosmic star formation history since z   5}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1703.09724},
 keywords = {galaxies: evolution, galaxies: star formation, cosmology: observations, radio continuum: galaxies},
     year = 2017,
    month = jun,
   volume = 602,
      eid = {A5},
    pages = {A5},
      doi = {10.1051/0004-6361/201629436},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...602A...5N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{delhaize17,
   author = {{Delhaize}, J. and {Smol{\v c}i{\'c}}, V. and {Delvecchio}, I. and 
	{Novak}, M. and {Sargent}, M. and {Baran}, N. and {Magnelli}, B. and 
	{Zamorani}, G. and {Schinnerer}, E. and {Murphy}, E.~J. and 
	{Aravena}, M. and {Berta}, S. and {Bondi}, M. and {Capak}, P. and 
	{Carilli}, C. and {Ciliegi}, P. and {Civano}, F. and {Ilbert}, O. and 
	{Karim}, A. and {Laigle}, C. and {Le F{\`e}vre}, O. and {Marchesi}, S. and 
	{McCracken}, H.~J. and {Salvato}, M. and {Seymour}, N. and {Tasca}, L.
	},
    title = "{The VLA-COSMOS 3 GHz Large Project: The infrared-radio correlation of star-forming galaxies and AGN to z {\lsim} 6}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1703.09723},
 keywords = {galaxies: evolution, galaxies: star formation, radio continuum: galaxies, infrared: galaxies},
     year = 2017,
    month = jun,
   volume = 602,
      eid = {A4},
    pages = {A4},
      doi = {10.1051/0004-6361/201629430},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...602A...4D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{delvecchio17,
   author = {{Delvecchio}, I. and {Smol{\v c}i{\'c}}, V. and {Zamorani}, G. and 
	{Lagos}, C.~D.~P. and {Berta}, S. and {Delhaize}, J. and {Baran}, N. and 
	{Alexander}, D.~M. and {Rosario}, D.~J. and {Gonzalez-Perez}, V. and 
	{Ilbert}, O. and {Lacey}, C.~G. and {Le F{\`e}vre}, O. and {Miettinen}, O. and 
	{Aravena}, M. and {Bondi}, M. and {Carilli}, C. and {Ciliegi}, P. and 
	{Mooley}, K. and {Novak}, M. and {Schinnerer}, E. and {Capak}, P. and 
	{Civano}, F. and {Fanidakis}, N. and {Herrera Ruiz}, N. and 
	{Karim}, A. and {Laigle}, C. and {Marchesi}, S. and {McCracken}, H.~J. and 
	{Middleberg}, E. and {Salvato}, M. and {Tasca}, L.},
    title = "{The VLA-COSMOS 3 GHz Large Project: AGN and host-galaxy properties out to z {\lsim} 6}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1703.09720},
 keywords = {radio continuum: galaxies, galaxies: nuclei, galaxies: active, galaxies: evolution},
     year = 2017,
    month = jun,
   volume = 602,
      eid = {A3},
    pages = {A3},
      doi = {10.1051/0004-6361/201629367},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...602A...3D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{smolcic17b,
   author = {{Smol{\v c}i{\'c}}, V. and {Delvecchio}, I. and {Zamorani}, G. and 
	{Baran}, N. and {Novak}, M. and {Delhaize}, J. and {Schinnerer}, E. and 
	{Berta}, S. and {Bondi}, M. and {Ciliegi}, P. and {Capak}, P. and 
	{Civano}, F. and {Karim}, A. and {Le Fevre}, O. and {Ilbert}, O. and 
	{Laigle}, C. and {Marchesi}, S. and {McCracken}, H.~J. and {Tasca}, L. and 
	{Salvato}, M. and {Vardoulaki}, E.},
    title = "{The VLA-COSMOS 3 GHz Large Project: Multiwavelength counterparts and the composition of the faint radio population}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1703.09719},
 keywords = {radio continuum: galaxies, catalogs},
     year = 2017,
    month = jun,
   volume = 602,
      eid = {A2},
    pages = {A2},
      doi = {10.1051/0004-6361/201630223},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...602A...2S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{smolcic17a,
   author = {{Smol{\v c}i{\'c}}, V. and {Novak}, M. and {Bondi}, M. and {Ciliegi}, P. and 
	{Mooley}, K.~P. and {Schinnerer}, E. and {Zamorani}, G. and 
	{Navarrete}, F. and {Bourke}, S. and {Karim}, A. and {Vardoulaki}, E. and 
	{Leslie}, S. and {Delhaize}, J. and {Carilli}, C.~L. and {Myers}, S.~T. and 
	{Baran}, N. and {Delvecchio}, I. and {Miettinen}, O. and {Banfield}, J. and 
	{Balokovi{\'c}}, M. and {Bertoldi}, F. and {Capak}, P. and {Frail}, D.~A. and 
	{Hallinan}, G. and {Hao}, H. and {Herrera Ruiz}, N. and {Horesh}, A. and 
	{Ilbert}, O. and {Intema}, H. and {Jeli{\'c}}, V. and {Kl{\"o}ckner}, H.-R. and 
	{Krpan}, J. and {Kulkarni}, S.~R. and {McCracken}, H. and {Laigle}, C. and 
	{Middleberg}, E. and {Murphy}, E.~J. and {Sargent}, M. and {Scoville}, N.~Z. and 
	{Sheth}, K.},
    title = "{The VLA-COSMOS 3 GHz Large Project: Continuum data and source catalog release}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1703.09713},
 keywords = {catalogs, cosmology: observations, radio continuum: galaxies},
     year = 2017,
    month = jun,
   volume = 602,
      eid = {A1},
    pages = {A1},
      doi = {10.1051/0004-6361/201628704},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...602A...1S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{smolcic09,
   author = {{Smol{\v c}i{\'c}}, V. and {Zamorani}, G. and {Schinnerer}, E. and 
	{Bardelli}, S. and {Bondi}, M. and {B{\^i}rzan}, L. and {Carilli}, C.~L. and 
	{Ciliegi}, P. and {Elvis}, M. and {Impey}, C.~D. and {Koekemoer}, A.~M. and 
	{Merloni}, A. and {Paglione}, T. and {Salvato}, M. and {Scodeggio}, M. and 
	{Scoville}, N. and {Trump}, J.~R.},
    title = "{Cosmic Evolution of Radio Selected Active Galactic Nuclei in the Cosmos Field}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0901.3372},
 primaryClass = "astro-ph.CO",
 keywords = {cosmology: observations, galaxies: active, galaxies: evolution, galaxies: fundamental parameters, radio continuum: galaxies},
     year = 2009,
    month = may,
   volume = 696,
    pages = {24-39},
      doi = {10.1088/0004-637X/696/1/24},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...696...24S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hb14,
   author = {{Heckman}, T.~M. and {Best}, P.~N.},
    title = "{The Coevolution of Galaxies and Supermassive Black Holes: Insights from Surveys of the Contemporary Universe}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1403.4620},
     year = 2014,
    month = aug,
   volume = 52,
    pages = {589-660},
      doi = {10.1146/annurev-astro-081913-035722},
   adsurl = {http://adsabs.harvard.edu/abs/2014ARA%26A..52..589H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bh12,
   author = {{Best}, P.~N. and {Heckman}, T.~M.},
    title = "{On the fundamental dichotomy in the local radio-AGN population: accretion, evolution and host galaxy properties}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1201.2397},
 keywords = {accretion, accretion discs, black hole physics, galaxies: active, galaxies: jets, radio continuum: galaxies},
     year = 2012,
    month = apr,
   volume = 421,
    pages = {1569-1582},
      doi = {10.1111/j.1365-2966.2012.20414.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.421.1569B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{herreraruiz16,
   author = {{Herrera Ruiz}, N. and {Middelberg}, E. and {Norris}, R.~P. and 
	{Maini}, A.},
    title = "{Unveiling the origin of the radio emission in radio-quiet quasars}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1603.07136},
 keywords = {galaxies: active, radio continuum: galaxies, quasars: general, galaxies: evolution},
     year = 2016,
    month = may,
   volume = 589,
      eid = {L2},
    pages = {L2},
      doi = {10.1051/0004-6361/201628302},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...589L...2H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{padovani15,
   author = {{Padovani}, P. and {Bonzini}, M. and {Kellermann}, K.~I. and 
	{Miller}, N. and {Mainieri}, V. and {Tozzi}, P.},
    title = "{Radio-faint AGN: a tale of two populations}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1506.06554},
 keywords = {surveys, galaxies: active, galaxies: evolution, quasars: general, galaxies: starburst, radio continuum: galaxies},
     year = 2015,
    month = sep,
   volume = 452,
    pages = {1263-1279},
      doi = {10.1093/mnras/stv1375},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.452.1263P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{filho06,
   author = {{Filho}, M.~E. and {Barthel}, P.~D. and {Ho}, L.~C.},
    title = "{A radio census of nuclear activity in nearby galaxies}",
  journal = {\aap},
   eprint = {astro-ph/0601080},
 keywords = {galaxies: active, galaxies: nuclei, galaxies: luminosity function, mass function},
     year = 2006,
    month = may,
   volume = 451,
    pages = {71-83},
      doi = {10.1051/0004-6361:20054510},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...451...71F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gendre13,
   author = {{Gendre}, M.~A. and {Best}, P.~N. and {Wall}, J.~V. and {Ker}, L.~M.
	},
    title = "{The relation between morphology, accretion modes and environmental factors in local radio AGN}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1301.1526},
 keywords = {catalogues, galaxies: active, galaxies: luminosity function, mass function, galaxies: statistics, radio continuum: galaxies},
     year = 2013,
    month = apr,
   volume = 430,
    pages = {3086-3101},
      doi = {10.1093/mnras/stt116},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.430.3086G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{best14,
   author = {{Best}, P.~N. and {Ker}, L.~M. and {Simpson}, C. and {Rigby}, E.~E. and 
	{Sabater}, J.},
    title = "{The cosmic evolution of radio-AGN feedback to z = 1}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1409.0263},
 keywords = {accretion, accretion discs, galaxies: active, galaxies: evolution, galaxies: jets, radio continuum: galaxies},
     year = 2014,
    month = nov,
   volume = 445,
    pages = {955-969},
      doi = {10.1093/mnras/stu1776},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.445..955B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pracy16,
   author = {{Pracy}, M.~B. and {Ching}, J.~H.~Y. and {Sadler}, E.~M. and 
	{Croom}, S.~M. and {Baldry}, I.~K. and {Bland-Hawthorn}, J. and 
	{Brough}, S. and {Brown}, M.~J.~I. and {Couch}, W.~J. and {Davis}, T.~M. and 
	{Drinkwater}, M.~J. and {Hopkins}, A.~M. and {Jarvis}, M.~J. and 
	{Jelliffe}, B. and {Jurek}, R.~J. and {Loveday}, J. and {Pimbblet}, K.~A. and 
	{Prescott}, M. and {Wisnioski}, E. and {Woods}, D.},
    title = "{GAMA/WiggleZ: the 1.4 GHz radio luminosity functions of high- and low-excitation radio galaxies and their redshift evolution to z = 0.75}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1604.04332},
 keywords = {galaxies: active, radio continuum: galaxies},
     year = 2016,
    month = jul,
   volume = 460,
    pages = {2-17},
      doi = {10.1093/mnras/stw910},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.460....2P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{croton06,
   author = {{Croton}, D.~J. and {Springel}, V. and {White}, S.~D.~M. and 
	{De Lucia}, G. and {Frenk}, C.~S. and {Gao}, L. and {Jenkins}, A. and 
	{Kauffmann}, G. and {Navarro}, J.~F. and {Yoshida}, N.},
    title = "{The many lives of active galactic nuclei: cooling flows, black holes and the luminosities and colours of galaxies}",
  journal = {\mnras},
   eprint = {astro-ph/0508046},
 keywords = {black hole physics, galaxies: active, cooling flows, galaxies: evolution, galaxies: formation, cosmology: theory},
     year = 2006,
    month = jan,
   volume = 365,
    pages = {11-28},
      doi = {10.1111/j.1365-2966.2005.09675.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.365...11C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bonzini13,
   author = {{Bonzini}, M. and {Padovani}, P. and {Mainieri}, V. and {Kellermann}, K.~I. and 
	{Miller}, N. and {Rosati}, P. and {Tozzi}, P. and {Vattakunnel}, S.
	},
    title = "{The sub-mJy radio sky in the Extended Chandra Deep Field-South: source population}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1310.1248},
 keywords = {catalogues, galaxies: active, galaxies: star formation},
     year = 2013,
    month = dec,
   volume = 436,
    pages = {3759-3771},
      doi = {10.1093/mnras/stt1879},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.436.3759B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{condon92,
   author = {{Condon}, J.~J.},
    title = "{Radio emission from normal galaxies}",
  journal = {\araa},
 keywords = {Cosmic Rays, Radio Emission, Radio Sources (Astronomy), Star Formation, Starburst Galaxies, Synchrotron Radiation, Black Holes (Astronomy), H Ii Regions, Infrared Radiation, Relativistic Particles},
     year = 1992,
   volume = 30,
    pages = {575-611},
      doi = {10.1146/annurev.aa.30.090192.003043},
   adsurl = {http://adsabs.harvard.edu/abs/1992ARA%26A..30..575C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{condon77,
   author = {{Condon}, J.~J. and {Hicks}, P.~D. and {Jauncey}, D.~L.},
    title = "{Optical identifications of Parkes sources with flat spectra.}",
  journal = {\aj},
     year = 1977,
    month = sep,
   volume = 82,
    pages = {692-700},
      doi = {10.1086/112109},
   adsurl = {http://adsabs.harvard.edu/abs/1977AJ.....82..692C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{laigle16,
   author = {{Laigle}, C. and {McCracken}, H.~J. and {Ilbert}, O. and {Hsieh}, B.~C. and 
	{Davidzon}, I. and {Capak}, P. and {Hasinger}, G. and {Silverman}, J.~D. and 
	{Pichon}, C. and {Coupon}, J. and {Aussel}, H. and {Le Borgne}, D. and 
	{Caputi}, K. and {Cassata}, P. and {Chang}, Y.-Y. and {Civano}, F. and 
	{Dunlop}, J. and {Fynbo}, J. and {Kartaltepe}, J.~S. and {Koekemoer}, A. and 
	{Le F{\`e}vre}, O. and {Le Floc'h}, E. and {Leauthaud}, A. and 
	{Lilly}, S. and {Lin}, L. and {Marchesi}, S. and {Milvang-Jensen}, B. and 
	{Salvato}, M. and {Sanders}, D.~B. and {Scoville}, N. and {Smolcic}, V. and 
	{Stockmann}, M. and {Taniguchi}, Y. and {Tasca}, L. and {Toft}, S. and 
	{Vaccari}, M. and {Zabl}, J.},
    title = "{The COSMOS2015 Catalog: Exploring the 1 $\lt$ z $\lt$ 6 Universe with Half a Million Galaxies}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1604.02350},
 keywords = {catalogs, galaxies: evolution, galaxies: high-redshift, galaxies: photometry, methods: observational, techniques: photometric},
     year = 2016,
    month = jun,
   volume = 224,
      eid = {24},
    pages = {24},
      doi = {10.3847/0067-0049/224/2/24},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJS..224...24L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{schinnerer07,
   author = {{Schinnerer}, E. and {Smol{\v c}i{\'c}}, V. and {Carilli}, C.~L. and 
	{Bondi}, M. and {Ciliegi}, P. and {Jahnke}, K. and {Scoville}, N.~Z. and 
	{Aussel}, H. and {Bertoldi}, F. and {Blain}, A.~W. and {Impey}, C.~D. and 
	{Koekemoer}, A.~M. and {Le Fevre}, O. and {Urry}, C.~M.},
    title = "{The VLA-COSMOS Survey. II. Source Catalog of the Large Project}",
  journal = {\apjs},
   eprint = {astro-ph/0612314},
 keywords = {Cosmology: Observations, Radio Continuum: Galaxies, Surveys},
     year = 2007,
    month = sep,
   volume = 172,
    pages = {46-69},
      doi = {10.1086/516587},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..172...46S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{schinnerer10,
   author = {{Schinnerer}, E. and {Sargent}, M.~T. and {Bondi}, M. and {Smol{\v c}i{\'c}}, V. and 
	{Datta}, A. and {Carilli}, C.~L. and {Bertoldi}, F. and {Blain}, A. and 
	{Ciliegi}, P. and {Koekemoer}, A. and {Scoville}, N.~Z.},
    title = "{The VLA-COSMOS Survey. IV. Deep Data and Joint Catalog}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1005.1641},
 keywords = {cosmology: observations, radio continuum: galaxies, surveys},
     year = 2010,
    month = jun,
   volume = 188,
    pages = {384-404},
      doi = {10.1088/0067-0049/188/2/384},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJS..188..384S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{donley12,
   author = {{Donley}, J.~L. and {Koekemoer}, A.~M. and {Brusa}, M. and {Capak}, P. and 
	{Cardamone}, C.~N. and {Civano}, F. and {Ilbert}, O. and {Impey}, C.~D. and 
	{Kartaltepe}, J.~S. and {Miyaji}, T. and {Salvato}, M. and {Sanders}, D.~B. and 
	{Trump}, J.~R. and {Zamorani}, G.},
    title = "{Identifying Luminous Active Galactic Nuclei in Deep Surveys: Revised IRAC Selection Criteria}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1201.3899},
 keywords = {galaxies: active, infrared: galaxies, X-rays: galaxies},
     year = 2012,
    month = apr,
   volume = 748,
      eid = {142},
    pages = {142},
      doi = {10.1088/0004-637X/748/2/142},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...748..142D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{schmidt68,
   author = {{Schmidt}, M.},
    title = "{Space Distribution and Luminosity Functions of Quasi-Stellar Radio Sources}",
  journal = {\apj},
     year = 1968,
    month = feb,
   volume = 151,
    pages = {393},
      doi = {10.1086/149446},
   adsurl = {http://adsabs.harvard.edu/abs/1968ApJ...151..393S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{becker94,
   author = {{Becker}, R.~H. and {White}, R.~L. and {Helfand}, D.~J.},
    title = "{The VLA's FIRST Survey}",
booktitle = {Astronomical Data Analysis Software and Systems III},
     year = 1994,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 61,
   editor = {{Crabtree}, D.~R. and {Hanisch}, R.~J. and {Barnes}, J.},
    pages = {165},
   adsurl = {http://adsabs.harvard.edu/abs/1994ASPC...61..165B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{whitaker12,
   author = {{Whitaker}, K.~E. and {van Dokkum}, P.~G. and {Brammer}, G. and 
	{Franx}, M.},
    title = "{The Star Formation Mass Sequence Out to z = 2.5}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1205.0547},
 keywords = {galaxies: evolution, galaxies: formation, galaxies: high-redshift},
     year = 2012,
    month = aug,
   volume = 754,
      eid = {L29},
    pages = {L29},
      doi = {10.1088/2041-8205/754/2/L29},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...754L..29W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{smolcic17c,
   author = {{Smol{\v c}i{\'c}}, V. and {Novak}, M. and {Delvecchio}, I. and 
	{Ceraj}, L. and {Bondi}, M. and {Delhaize}, J. and {Marchesi}, S. and 
	{Murphy}, E. and {Schinnerer}, E. and {Vardoulaki}, E. and {Zamorani}, G.
	},
    title = "{The VLA-COSMOS 3 GHz Large Project: Cosmic evolution of radio AGN and implications for radio-mode feedback since z   5}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1705.07090},
 keywords = {surveys, radio continuum: galaxies, galaxies: evolution},
     year = 2017,
    month = jun,
   volume = 602,
      eid = {A6},
    pages = {A6},
      doi = {10.1051/0004-6361/201730685},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...602A...6S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ms07,
   author = {{Mauch}, T. and {Sadler}, E.~M.},
    title = "{Radio sources in the 6dFGS: local luminosity functions at 1.4GHz for star-forming galaxies and radio-loud AGN}",
  journal = {\mnras},
   eprint = {astro-ph/0612018},
 keywords = {surveys, galaxies: active, galaxies: luminosity function, mass function, galaxies: starburst, radio continuum: galaxies},
     year = 2007,
    month = mar,
   volume = 375,
    pages = {931-950},
      doi = {10.1111/j.1365-2966.2006.11353.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.375..931M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fanidakis11,
   author = {{Fanidakis}, N. and {Baugh}, C.~M. and {Benson}, A.~J. and {Bower}, R.~G. and 
	{Cole}, S. and {Done}, C. and {Frenk}, C.~S.},
    title = "{Grand unification of AGN activity in the {$\Lambda$}CDM cosmology}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0911.1128},
 keywords = {methods: numerical, galaxies: active, galaxies: jets, galaxies: nuclei, quasars: general},
     year = 2011,
    month = jan,
   volume = 410,
    pages = {53-74},
      doi = {10.1111/j.1365-2966.2010.17427.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.410...53F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{fb99,
   author = {{Falcke}, H. and {Biermann}, P.~L.},
    title = "{The jet/disk symbiosis. III. What the radio cores in GRS 1915+105, NGC 4258, M 81 and SGR A* tell us about accreting black holes}",
  journal = {\aap},
   eprint = {astro-ph/9810226},
 keywords = {ACCRETION, ACCRETION DISKS, STARS: INDIVIDUAL: GRS 1915+105, GALAXY: CENTER, GALAXIES: INDIVIDUAL: M 81, GALAXIES: INDIVIDUAL: NGC 4258, GALAXIES: JETS},
     year = 1999,
    month = feb,
   volume = 342,
    pages = {49-56},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...342...49F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{croton16,
   author = {{Croton}, D.~J. and {Stevens}, A.~R.~H. and {Tonini}, C. and 
	{Garel}, T. and {Bernyk}, M. and {Bibiano}, A. and {Hodkinson}, L. and 
	{Mutch}, S.~J. and {Poole}, G.~B. and {Shattow}, G.~M.},
    title = "{Semi-Analytic Galaxy Evolution (SAGE): Model Calibration and Basic Results}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1601.04709},
 keywords = {galaxies: active, galaxies: evolution, galaxies: halos, methods: numerical},
     year = 2016,
    month = feb,
   volume = 222,
      eid = {22},
    pages = {22},
      doi = {10.3847/0067-0049/222/2/22},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJS..222...22C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{herreraruiz17,
   author = {{Herrera Ruiz}, N. and {Middelberg}, E. and {Deller}, A. and 
	{Norris}, R.~P. and {Best}, P.~N. and {Brisken}, W. and {Schinnerer}, E. and 
	{Smol{\v c}i{\'c}}, V. and {Delvecchio}, I. and {Momjian}, E. and 
	{Bomans}, D. and {Scoville}, N.~Z. and {Carilli}, C.},
    title = "{The faint radio sky: VLBA observations of the COSMOS field}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1707.07512},
 keywords = {catalogs, galaxies: active, radio continuum: galaxies},
     year = 2017,
    month = nov,
   volume = 607,
      eid = {A132},
    pages = {A132},
      doi = {10.1051/0004-6361/201731163},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...607A.132H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gehrels86,
   author = {{Gehrels}, N.},
    title = "{Confidence limits for small numbers of events in astrophysical data}",
  journal = {\apj},
 keywords = {Astrophysics, Binomial Theorem, Confidence Limits, Data Processing, Poisson Density Functions, Approximation, Tables (Data)},
     year = 1986,
    month = apr,
   volume = 303,
    pages = {336-346},
      doi = {10.1086/164079},
   adsurl = {http://adsabs.harvard.edu/abs/1986ApJ...303..336G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{magorrian98,
   author = {{Magorrian}, J. and {Tremaine}, S. and {Richstone}, D. and {Bender}, R. and 
	{Bower}, G. and {Dressler}, A. and {Faber}, S.~M. and {Gebhardt}, K. and 
	{Green}, R. and {Grillmair}, C. and {Kormendy}, J. and {Lauer}, T.
	},
    title = "{The Demography of Massive Dark Objects in Galaxy Centers}",
  journal = {\aj},
   eprint = {astro-ph/9708072},
 keywords = {COSMOLOGY: DARK MATTER, GALAXIES: NUCLEI},
     year = 1998,
    month = jun,
   volume = 115,
    pages = {2285-2305},
      doi = {10.1086/300353},
   adsurl = {http://adsabs.harvard.edu/abs/1998AJ....115.2285M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fm00,
   author = {{Ferrarese}, L. and {Merritt}, D.},
    title = "{A Fundamental Relation between Supermassive Black Holes and Their Host Galaxies}",
  journal = {\apjl},
   eprint = {astro-ph/0006053},
 keywords = {Black Hole Physics, Galaxies: Evolution, Galaxies: Kinematics and Dynamics},
     year = 2000,
    month = aug,
   volume = 539,
    pages = {L9-L12},
      doi = {10.1086/312838},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...539L...9F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{best05,
   author = {{Best}, P.~N. and {Kauffmann}, G. and {Heckman}, T.~M. and {Ivezi{\'c}}, {\v Z}.
	},
    title = "{A sample of radio-loud active galactic nuclei in the Sloan Digital Sky Survey}",
  journal = {\mnras},
   eprint = {astro-ph/0506268},
 keywords = {surveys, galaxies: active, galaxies: evolution, galaxies: luminosity function, mass function, galaxies: starburst, radio continuum: galaxies},
     year = 2005,
    month = sep,
   volume = 362,
    pages = {9-24},
      doi = {10.1111/j.1365-2966.2005.09283.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.362....9B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sadler02,
   author = {{Sadler}, E.~M. and {Jackson}, C.~A. and {Cannon}, R.~D. and 
	{McIntyre}, V.~J. and {Murphy}, T. and {Bland-Hawthorn}, J. and 
	{Bridges}, T. and {Cole}, S. and {Colless}, M. and {Collins}, C. and 
	{Couch}, W. and {Dalton}, G. and {De Propris}, R. and {Driver}, S.~P. and 
	{Efstathiou}, G. and {Ellis}, R.~S. and {Frenk}, C.~S. and {Glazebrook}, K. and 
	{Lahav}, O. and {Lewis}, I. and {Lumsden}, S. and {Maddox}, S. and 
	{Madgwick}, D. and {Norberg}, P. and {Peacock}, J.~A. and {Peterson}, B.~A. and 
	{Sutherland}, W. and {Taylor}, K.},
    title = "{Radio sources in the 2dF Galaxy Redshift Survey - II. Local radio luminosity functions for AGN and star-forming galaxies at 1.4 GHz}",
  journal = {\mnras},
   eprint = {astro-ph/0106173},
 keywords = {GALAXIES: ACTIVE, GALAXIES: LUMINOSITY FUNCTION, MASS FUNCTION, GALAXIES: STARBURST, RADIO CONTINUUM: GALAXIES},
     year = 2002,
    month = jan,
   volume = 329,
    pages = {227-245},
      doi = {10.1046/j.1365-8711.2002.04998.x},
   adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.329..227S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ah12,
   author = {{Alexander}, D.~M. and {Hickox}, R.~C.},
    title = "{What drives the growth of black holes?}",
  journal = {\nar},
archivePrefix = "arXiv",
   eprint = {1112.1949},
     year = 2012,
    month = jun,
   volume = 56,
    pages = {93-121},
      doi = {10.1016/j.newar.2011.11.003},
   adsurl = {http://adsabs.harvard.edu/abs/2012NewAR..56...93A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lusso12,
   author = {{Lusso}, E. and {Comastri}, A. and {Simmons}, B.~D. and {Mignoli}, M. and 
	{Zamorani}, G. and {Vignali}, C. and {Brusa}, M. and {Shankar}, F. and 
	{Lutz}, D. and {Trump}, J.~R. and {Maiolino}, R. and {Gilli}, R. and 
	{Bolzonella}, M. and {Puccetti}, S. and {Salvato}, M. and {Impey}, C.~D. and 
	{Civano}, F. and {Elvis}, M. and {Mainieri}, V. and {Silverman}, J.~D. and 
	{Koekemoer}, A.~M. and {Bongiorno}, A. and {Merloni}, A. and 
	{Berta}, S. and {Le Floc'h}, E. and {Magnelli}, B. and {Pozzi}, F. and 
	{Riguccini}, L.},
    title = "{Bolometric luminosities and Eddington ratios of X-ray selected active galactic nuclei in the XMM-COSMOS survey}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1206.2642},
 keywords = {methods: statistical, galaxies: active, galaxies: evolution, quasars: general },
     year = 2012,
    month = sep,
   volume = 425,
    pages = {623-640},
      doi = {10.1111/j.1365-2966.2012.21513.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.425..623L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bower06,
   author = {{Bower}, R.~G. and {Benson}, A.~J. and {Malbon}, R. and {Helly}, J.~C. and 
	{Frenk}, C.~S. and {Baugh}, C.~M. and {Cole}, S. and {Lacey}, C.~G.
	},
    title = "{Breaking the hierarchy of galaxy formation}",
  journal = {\mnras},
   eprint = {astro-ph/0511338},
 keywords = {galaxies: evolution: galaxies: formation: galaxies: luminosity function, galaxies: evolution, galaxies: formation, galaxies: luminosity function},
     year = 2006,
    month = aug,
   volume = 370,
    pages = {645-655},
      doi = {10.1111/j.1365-2966.2006.10519.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.370..645B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ah12,
   author = {{Alexander}, D.~M. and {Hickox}, R.~C.},
    title = "{What drives the growth of black holes?}",
  journal = {\nar},
archivePrefix = "arXiv",
   eprint = {1112.1949},
     year = 2012,
    month = jun,
   volume = 56,
    pages = {93-121},
      doi = {10.1016/j.newar.2011.11.003},
   adsurl = {http://adsabs.harvard.edu/abs/2012NewAR..56...93A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fabian12,
   author = {{Fabian}, A.~C.},
    title = "{Observational Evidence of Active Galactic Nuclei Feedback}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1204.4114},
     year = 2012,
    month = sep,
   volume = 50,
    pages = {455-489},
      doi = {10.1146/annurev-astro-081811-125521},
   adsurl = {http://adsabs.harvard.edu/abs/2012ARA%26A..50..455F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ss73,
   author = {{Shakura}, N.~I. and {Sunyaev}, R.~A.},
    title = "{Black holes in binary systems. Observational appearance.}",
  journal = {\aap},
     year = 1973,
   volume = 24,
    pages = {337-355},
   adsurl = {http://adsabs.harvard.edu/abs/1973A%26A....24..337S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ny94,
   author = {{Narayan}, R. and {Yi}, I.},
    title = "{Advection-dominated accretion: A self-similar solution}",
  journal = {\apjl},
   eprint = {astro-ph/9403052},
 keywords = {Accretion Disks, Advection, Astronomical Models, Black Holes (Astronomy), Cooling Flows (Astrophysics), Stellar Mass Accretion, Viscous Flow, Hydrodynamics, Rotating Disks, Two Dimensional Flow},
     year = 1994,
    month = jun,
   volume = 428,
    pages = {L13-L16},
      doi = {10.1086/187381},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...428L..13N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ny95,
   author = {{Narayan}, R. and {Yi}, I.},
    title = "{Advection-dominated accretion: Self-similarity and bipolar outflows}",
  journal = {\apj},
   eprint = {astro-ph/9411058},
 keywords = {Accretion Disks, Advection, Analogies, Axisymmetric Flow, Bipolarity, Computational Astrophysics, Flow Equations, Viscous Flow, Approximation, Convection, Flow Characteristics, Hydrodynamics, Interstellar Matter, Stellar Rotation, Viscosity},
     year = 1995,
    month = may,
   volume = 444,
    pages = {231-243},
      doi = {10.1086/175599},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...444..231N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{cavagnolo10,
   author = {{Cavagnolo}, K.~W. and {McNamara}, B.~R. and {Nulsen}, P.~E.~J. and 
	{Carilli}, C.~L. and {Jones}, C. and {B{\^i}rzan}, L.},
    title = "{A Relationship Between AGN Jet Power and Radio Power}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1006.5699},
 keywords = {galaxies: active, galaxies: clusters: general, radio continuum: galaxies, X-rays: galaxies},
     year = 2010,
    month = sep,
   volume = 720,
    pages = {1066-1072},
      doi = {10.1088/0004-637X/720/2/1066},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...720.1066C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gs16,
   author = {{Godfrey}, L.~E.~H. and {Shabala}, S.~S.},
    title = "{Mutual distance dependence drives the observed jet-power-radio-luminosity scaling relations in radio galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1511.06007},
 keywords = {galaxies: active, galaxies: jets, radio continuum: galaxies},
     year = 2016,
    month = feb,
   volume = 456,
    pages = {1172-1184},
      doi = {10.1093/mnras/stv2712},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.456.1172G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{steinhardt14,
   author = {{Steinhardt}, C.~L. and {Speagle}, J.~S. and {Capak}, P. and 
	{Silverman}, J.~D. and {Carollo}, M. and {Dunlop}, J. and {Hashimoto}, Y. and 
	{Hsieh}, B.-C. and {Ilbert}, O. and {Le Fevre}, O. and {Le Floc'h}, E. and 
	{Lee}, N. and {Lin}, L. and {Lin}, Y.-T. and {Masters}, D. and 
	{McCracken}, H.~J. and {Nagao}, T. and {Petric}, A. and {Salvato}, M. and 
	{Sanders}, D. and {Scoville}, N. and {Sheth}, K. and {Strauss}, M.~A. and 
	{Taniguchi}, Y.},
    title = "{Star Formation at 4 $\lt$ z $\lt$ 6 from the Spitzer Large Area Survey with Hyper-Suprime-Cam (SPLASH)}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1407.7030},
 keywords = {galaxies: evolution},
     year = 2014,
    month = aug,
   volume = 791,
      eid = {L25},
    pages = {L25},
      doi = {10.1088/2041-8205/791/2/L25},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...791L..25S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{civano16,
   author = {{Civano}, F. and {Marchesi}, S. and {Comastri}, A. and {Urry}, M.~C. and 
	{Elvis}, M. and {Cappelluti}, N. and {Puccetti}, S. and {Brusa}, M. and 
	{Zamorani}, G. and {Hasinger}, G. and {Aldcroft}, T. and {Alexander}, D.~M. and 
	{Allevato}, V. and {Brunner}, H. and {Capak}, P. and {Finoguenov}, A. and 
	{Fiore}, F. and {Fruscione}, A. and {Gilli}, R. and {Glotfelty}, K. and 
	{Griffiths}, R.~E. and {Hao}, H. and {Harrison}, F.~A. and {Jahnke}, K. and 
	{Kartaltepe}, J. and {Karim}, A. and {LaMassa}, S.~M. and {Lanzuisi}, G. and 
	{Miyaji}, T. and {Ranalli}, P. and {Salvato}, M. and {Sargent}, M. and 
	{Scoville}, N.~J. and {Schawinski}, K. and {Schinnerer}, E. and 
	{Silverman}, J. and {Smolcic}, V. and {Stern}, D. and {Toft}, S. and 
	{Trakhtenbrot}, B. and {Treister}, E. and {Vignali}, C.},
    title = "{The Chandra Cosmos Legacy Survey: Overview and Point Source Catalog}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1601.00941},
 keywords = {catalogs, cosmology: observations, galaxies: evolution, quasars: general, surveys, X-rays: general},
     year = 2016,
    month = mar,
   volume = 819,
      eid = {62},
    pages = {62},
      doi = {10.3847/0004-637X/819/1/62},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...819...62C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{marchesi16,
   author = {{Marchesi}, S. and {Civano}, F. and {Elvis}, M. and {Salvato}, M. and 
	{Brusa}, M. and {Comastri}, A. and {Gilli}, R. and {Hasinger}, G. and 
	{Lanzuisi}, G. and {Miyaji}, T. and {Treister}, E. and {Urry}, C.~M. and 
	{Vignali}, C. and {Zamorani}, G. and {Allevato}, V. and {Cappelluti}, N. and 
	{Cardamone}, C. and {Finoguenov}, A. and {Griffiths}, R.~E. and 
	{Karim}, A. and {Laigle}, C. and {LaMassa}, S.~M. and {Jahnke}, K. and 
	{Ranalli}, P. and {Schawinski}, K. and {Schinnerer}, E. and 
	{Silverman}, J.~D. and {Smolcic}, V. and {Suh}, H. and {Trakhtenbrot}, B.
	},
    title = "{The Chandra COSMOS Legacy survey: optical/IR identifications}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1512.01105},
 keywords = {catalogs, cosmology: observations, galaxies: active, galaxies: evolution, surveys, X-rays: general},
     year = 2016,
    month = jan,
   volume = 817,
      eid = {34},
    pages = {34},
      doi = {10.3847/0004-637X/817/1/34},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...817...34M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{marshall85,
   author = {{Marshall}, H.~L.},
    title = "{The evolution of optically selected quasars with Z less than 2.2 and B less than 20}",
  journal = {\apj},
 keywords = {Luminosity, Quasars, Red Shift, Cosmology, Evolution (Development), Ultraviolet Astronomy},
     year = 1985,
    month = dec,
   volume = 299,
    pages = {109-121},
      doi = {10.1086/163685},
   adsurl = {http://adsabs.harvard.edu/abs/1985ApJ...299..109M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{brinchmann04,
   author = {{Brinchmann}, J. and {Charlot}, S. and {White}, S.~D.~M. and 
	{Tremonti}, C. and {Kauffmann}, G. and {Heckman}, T. and {Brinkmann}, J.
	},
    title = "{The physical properties of star-forming galaxies in the low-redshift Universe}",
  journal = {\mnras},
   eprint = {astro-ph/0311060},
 keywords = {surveys, galaxies: abundances, galaxies: evolution, galaxies: fundamental parameters, galaxies: general},
     year = 2004,
    month = jul,
   volume = 351,
    pages = {1151-1179},
      doi = {10.1111/j.1365-2966.2004.07881.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2004MNRAS.351.1151B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{salim07,
   author = {{Salim}, S. and {Rich}, R.~M. and {Charlot}, S. and {Brinchmann}, J. and 
	{Johnson}, B.~D. and {Schiminovich}, D. and {Seibert}, M. and 
	{Mallery}, R. and {Heckman}, T.~M. and {Forster}, K. and {Friedman}, P.~G. and 
	{Martin}, D.~C. and {Morrissey}, P. and {Neff}, S.~G. and {Small}, T. and 
	{Wyder}, T.~K. and {Bianchi}, L. and {Donas}, J. and {Lee}, Y.-W. and 
	{Madore}, B.~F. and {Milliard}, B. and {Szalay}, A.~S. and {Welsh}, B.~Y. and 
	{Yi}, S.~K.},
    title = "{UV Star Formation Rates in the Local Universe}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {0704.3611},
 keywords = {Galaxies: Active, Galaxies: Evolution, Galaxies: Fundamental Parameters, Surveys, Ultraviolet: Galaxies},
     year = 2007,
    month = dec,
   volume = 173,
    pages = {267-292},
      doi = {10.1086/519218},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..173..267S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{king08,
   author = {{King}, A.},
    title = "{Accretion in AGN: evolution of black hole mass and spin.}",
  journal = {\memsai},
 keywords = {accretion, quasars: general, galaxies: formation, nuclei, black hole physics},
     year = 2008,
   volume = 79,
    pages = {1066},
   adsurl = {http://adsabs.harvard.edu/abs/2008MmSAI..79.1066K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{fanidakis12,
   author = {{Fanidakis}, N. and {Baugh}, C.~M. and {Benson}, A.~J. and {Bower}, R.~G. and 
	{Cole}, S. and {Done}, C. and {Frenk}, C.~S. and {Hickox}, R.~C. and 
	{Lacey}, C. and {Del P.~Lagos}, C.},
    title = "{The evolution of active galactic nuclei across cosmic time: what is downsizing?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1011.5222},
 keywords = {methods: numerical, galaxies: active, galaxies: nuclei, quasars: general},
     year = 2012,
    month = feb,
   volume = 419,
    pages = {2797-2820},
      doi = {10.1111/j.1365-2966.2011.19931.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.419.2797F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lacey16,
   author = {{Lacey}, C.~G. and {Baugh}, C.~M. and {Frenk}, C.~S. and {Benson}, A.~J. and 
	{Bower}, R.~G. and {Cole}, S. and {Gonzalez-Perez}, V. and {Helly}, J.~C. and 
	{Lagos}, C.~D.~P. and {Mitchell}, P.~D.},
    title = "{A unified multiwavelength model of galaxy formation}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1509.08473},
 keywords = {galaxies: evolution, galaxies: formation, galaxies: high-redshift},
     year = 2016,
    month = nov,
   volume = 462,
    pages = {3854-3911},
      doi = {10.1093/mnras/stw1888},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.462.3854L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{fd81a,
   author = {{Freedman}, D. and {Diaconis}, P.},
    title = "{On the histogram as a density estimator: $L_2$ theory}",
  journal = {Probability Theory and Related Fields},
   eprint = {1509.08473},
 keywords = {citeulike:6360487},
     year = 1981,
    month = dec,
   volume = 57,
    pages = {453-476},
      doi = {10.1007/BF01025868}
}

@ARTICLE{miller93,
   author = {{Miller}, P. and {Rawlings}, S. and {Saunders}, R.},
    title = "{The Radio and Optical Properties of the Z$\lt$0.5 BQS Quasars}",
  journal = {\mnras},
     year = 1993,
    month = jul,
   volume = 263,
    pages = {425},
      doi = {10.1093/mnras/263.2.425},
   adsurl = {http://adsabs.harvard.edu/abs/1993MNRAS.263..425M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{yun01,
   author = {{Yun}, M.~S. and {Reddy}, N.~A. and {Condon}, J.~J.},
    title = "{Radio Properties of Infrared-selected Galaxies in the IRAS 2 Jy Sample}",
  journal = {\apj},
   eprint = {astro-ph/0102154},
 keywords = {Galaxies: Active, Galaxies: Luminosity Function, Mass Function, Galaxies: Starburst, Infrared: Galaxies, Radio Continuum: Galaxies, Surveys},
     year = 2001,
    month = jun,
   volume = 554,
    pages = {803-822},
      doi = {10.1086/323145},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...554..803Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bell03,
   author = {{Bell}, E.~F.},
    title = "{Estimating Star Formation Rates from Infrared and Radio Luminosities: The Origin of the Radio-Infrared Correlation}",
  journal = {\apj},
   eprint = {astro-ph/0212121},
 keywords = {ISM: Cosmic Rays, ISM: Dust, Extinction, Galaxies: General, Infrared: Galaxies, Radio Continuum: Galaxies, Ultraviolet: Galaxies},
     year = 2003,
    month = apr,
   volume = 586,
    pages = {794-813},
      doi = {10.1086/367829},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...586..794B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{magnelli15,
   author = {{Magnelli}, B. and {Ivison}, R.~J. and {Lutz}, D. and {Valtchanov}, I. and 
	{Farrah}, D. and {Berta}, S. and {Bertoldi}, F. and {Bock}, J. and 
	{Cooray}, A. and {Ibar}, E. and {Karim}, A. and {Le Floc'h}, E. and 
	{Nordon}, R. and {Oliver}, S.~J. and {Page}, M. and {Popesso}, P. and 
	{Pozzi}, F. and {Rigopoulou}, D. and {Riguccini}, L. and {Rodighiero}, G. and 
	{Rosario}, D. and {Roseboom}, I. and {Wang}, L. and {Wuyts}, S.
	},
    title = "{The far-infrared/radio correlation and radio spectral index of galaxies in the SFR-M$_{∗}$ plane up to z\~{}2}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1410.7412},
 keywords = {galaxies: evolution, galaxies: formation, galaxies:, starburst, galaxies: high-redshift, infrared: galaxies},
     year = 2015,
    month = jan,
   volume = 573,
      eid = {A45},
    pages = {A45},
      doi = {10.1051/0004-6361/201424937},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...573A..45M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{novak18,
   author = {{Novak}, M. and {Smolcic}, V. and {Schinnerer}, E. and {Zamorani}, G. and 
	{Delvecchio}, I. and {Bondi}, M. and {Delhaize}, J.},
    title = "{Constraints on submicrojansky radio number counts based on evolving VLA-COSMOS luminosity functions}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1803.01569},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2018,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180301569N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{guzzo07,
   author = {{Guzzo}, L. and {Cassata}, P. and {Finoguenov}, A. and {Massey}, R. and 
	{Scoville}, N.~Z. and {Capak}, P. and {Ellis}, R.~S. and {Mobasher}, B. and 
	{Taniguchi}, Y. and {Thompson}, D. and {Ajiki}, M. and {Aussel}, H. and 
	{B{\"o}hringer}, H. and {Brusa}, M. and {Calzetti}, D. and {Comastri}, A. and 
	{Franceschini}, A. and {Hasinger}, G. and {Kasliwal}, M.~M. and 
	{Kitzbichler}, M.~G. and {Kneib}, J.-P. and {Koekemoer}, A. and 
	{Leauthaud}, A. and {McCracken}, H.~J. and {Murayama}, T. and 
	{Nagao}, T. and {Rhodes}, J. and {Sanders}, D.~B. and {Sasaki}, S. and 
	{Shioya}, Y. and {Tasca}, L. and {Taylor}, J.~E.},
    title = "{The Cosmic Evolution Survey (COSMOS): A Large-Scale Structure at z=0.73 and the Relation of Galaxy Morphologies to Local Environment}",
  journal = {\apjs},
   eprint = {astro-ph/0701482},
 keywords = {Galaxies: Clusters: General, Galaxies: Evolution, Cosmology: Large-Scale Structure of Universe, Surveys},
     year = 2007,
    month = sep,
   volume = 172,
    pages = {254-269},
      doi = {10.1086/516588},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..172..254G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{iovino16,
   author = {{Iovino}, A. and {Petropoulou}, V. and {Scodeggio}, M. and {Bolzonella}, M. and 
	{Zamorani}, G. and {Bardelli}, S. and {Cucciati}, O. and {Pozzetti}, L. and 
	{Tasca}, L. and {Vergani}, D. and {Zucca}, E. and {Finoguenov}, A. and 
	{Ilbert}, O. and {Tanaka}, M. and {Salvato}, M. and {Kova{\v c}}, K. and 
	{Cassata}, P.},
    title = "{A high definition view of the COSMOS Wall at z \~{} 0.73}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1606.06185},
 keywords = {galaxies: evolution, galaxies: groups: general, large-scale structure of Universe},
     year = 2016,
    month = aug,
   volume = 592,
      eid = {A78},
    pages = {A78},
      doi = {10.1051/0004-6361/201527673},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...592A..78I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bz77,
   author = {{Blandford}, R.~D. and {Znajek}, R.~L.},
    title = "{Electromagnetic extraction of energy from Kerr black holes}",
  journal = {\mnras},
 keywords = {Black Holes (Astronomy), Electromagnetic Fields, Energy Sources, Rotating Matter, Active Galactic Nuclei, Astrophysics, Electron-Positron Pairs, Pair Production},
     year = 1977,
    month = may,
   volume = 179,
    pages = {433-456},
      doi = {10.1093/mnras/179.3.433},
   adsurl = {http://adsabs.harvard.edu/abs/1977MNRAS.179..433B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{o'sullivan11,
   author = {{O'Sullivan}, E. and {Giacintucci}, S. and {David}, L.~P. and 
	{Gitti}, M. and {Vrtilek}, J.~M. and {Raychaudhury}, S. and 
	{Ponman}, T.~J.},
    title = "{Heating the Hot Atmospheres of Galaxy Groups and Clusters with Cavities: The Relationship between Jet Power and Low-frequency Radio Emission}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1104.2411},
 keywords = {galaxies: active, galaxies: clusters: general, galaxies: clusters: intracluster medium, galaxies: groups: general, X-rays: galaxies: clusters},
     year = 2011,
    month = jul,
   volume = 735,
      eid = {11},
    pages = {11},
      doi = {10.1088/0004-637X/735/1/11},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...735...11O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{birzan04,
   author = {{B{\^i}rzan}, L. and {Rafferty}, D.~A. and {McNamara}, B.~R. and 
	{Wise}, M.~W. and {Nulsen}, P.~E.~J.},
    title = "{A Systematic Study of Radio-induced X-Ray Cavities in Clusters, Groups, and Galaxies}",
  journal = {\apj},
   eprint = {astro-ph/0402348},
 keywords = {Galaxies: Active, Galaxies: Clusters: General, X-Rays: Galaxies, X-Rays: Galaxies: Clusters},
     year = 2004,
    month = jun,
   volume = 607,
    pages = {800-809},
      doi = {10.1086/383519},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...607..800B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sargent10,
   author = {{Sargent}, M.~T. and {Schinnerer}, E. and {Murphy}, E. and {Aussel}, H. and 
	{Le Floc'h}, E. and {Frayer}, D.~T. and {Mart{\'{\i}}nez-Sansigre}, A. and 
	{Oesch}, P. and {Salvato}, M. and {Smol{\v c}i{\'c}}, V. and 
	{Zamorani}, G. and {Brusa}, M. and {Cappelluti}, N. and {Carilli}, C.~L. and 
	{Carollo}, C.~M. and {Ilbert}, O. and {Kartaltepe}, J. and {Koekemoer}, A.~M. and 
	{Lilly}, S.~J. and {Sanders}, D.~B. and {Scoville}, N.~Z.},
    title = "{The VLA-COSMOS Perspective on the Infrared-Radio Relation. I. New Constraints on Selection Biases and the Non-Evolution of the Infrared/Radio Properties of Star-Forming and Active Galactic Nucleus Galaxies at Intermediate and High Redshift}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1001.1354},
 keywords = {cosmology: observations, galaxies: active, galaxies: evolution, galaxies: high-redshift, infrared: galaxies, radio continuum: galaxies, surveys},
     year = 2010,
    month = feb,
   volume = 186,
    pages = {341-377},
      doi = {10.1088/0067-0049/186/2/341},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJS..186..341S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> tab_alpha_evol.tex <==
$0.36$ & 3.68 $\pm 0.61$ & 5.57$\pm 0.91$\\

$0.65$ & 2.57 $\pm 0.40$ & 3.89$\pm 0.61$ \\

$0.82$ & 3.24$\pm 0.19$ & 4.90 $\pm 0.28$ \\

$0.98$ & 2.45 $\pm 0.29$ & 3.66 $\pm 0.34$ \\

$1.23$ & 2.21 $\pm 0.35$ & 3.29 $\pm 0.37$ \\

$1.53$ & 2.09 $\pm 0.27$ & 3.14 $\pm 0.38$ \\

$1.89$ & 1.67 $\pm 0.14$ & 2.51 $\pm 0.21$ \\

$2.46$ & 1.30 $\pm 0.13$ & 1.92 $\pm 0.12$ \\

$3.35$ & 0.22 $\pm 0.26$ & 0.32 $\pm 0.35$ \\


==> tab_lumfun_vmax1.tex <==
$0.1<z<0.4$ & 21.77$_{-1.1}^{+0.23}$ & -2.85$_{-0.077}^{+0.094}$ & 189 \\
 & 22.15$_{-0.15}^{+0.18}$ & -2.88$_{-0.029}^{+0.031}$ & 217 \\
 & 22.46$_{-0.14}^{+0.19}$ & -3.12$_{-0.034}^{+0.037}$ & 149 \\
 & 22.77$_{-0.12}^{+0.20}$ & -3.55$_{-0.055}^{+0.063}$ & 56 \\
 & 23.09$_{-0.12}^{+0.21}$ & -4.05$_{-0.090}^{+0.11}$ & 19 \\
 & 23.34$_{-0.048}^{+0.28}$ & -4.63$_{-0.22}^{+0.25}$ & 5 \\
$0.4<z<0.6$ & 22.29$_{-0.31}^{+0.11}$ & -2.97$_{-0.046}^{+0.052}$ & 142 \\
 & 22.54$_{-0.14}^{+0.13}$ & -3.19$_{-0.033}^{+0.036}$ & 160 \\
 & 22.80$_{-0.12}^{+0.15}$ & -3.33$_{-0.035}^{+0.038}$ & 143 \\
 & 23.04$_{-0.090}^{+0.18}$ & -3.67$_{-0.052}^{+0.059}$ & 65 \\
 & 23.31$_{-0.096}^{+0.18}$ & -4.32$_{-0.097}^{+0.12}$ & 16 \\
 & 23.68$_{-0.19}^{+0.081}$ & -5.05$_{-0.30}^{+0.34}$ & 3 \\
$0.6<z<0.8$ & 22.61$_{-0.23}^{+0.080}$ & -2.89$_{-0.075}^{+0.091}$ & 179 \\
 & 22.84$_{-0.15}^{+0.15}$ & -3.13$_{-0.025}^{+0.027}$ & 283 \\
 & 23.11$_{-0.12}^{+0.17}$ & -3.47$_{-0.033}^{+0.035}$ & 165 \\
 & 23.40$_{-0.12}^{+0.17}$ & -3.99$_{-0.057}^{+0.066}$ & 51 \\
 & 23.71$_{-0.13}^{+0.16}$ & -4.68$_{-0.11}^{+0.16}$ & 11 \\
 & 24.06$_{-0.19}^{+0.10}$ & -5.43$_{-0.37}^{+0.45}$ & 2 \\
$0.8<z<1.0$ & 22.85$_{-0.17}^{+0.074}$ & -3.01$_{-0.041}^{+0.046}$ & 172 \\
 & 23.05$_{-0.13}^{+0.13}$ & -3.13$_{-0.024}^{+0.025}$ & 312 \\
 & 23.30$_{-0.12}^{+0.14}$ & -3.45$_{-0.030}^{+0.032}$ & 198 \\
 & 23.54$_{-0.099}^{+0.16}$ & -3.85$_{-0.046}^{+0.051}$ & 82 \\
 & 23.81$_{-0.11}^{+0.15}$ & -4.31$_{-0.073}^{+0.088}$ & 30 \\
 & 24.11$_{-0.15}^{+0.11}$ & -4.89$_{-0.17}^{+0.18}$ & 8 \\
$1.0<z<1.3$ & 23.10$_{-0.21}^{+0.081}$ & -3.19$_{-0.046}^{+0.052}$ & 216 \\
 & 23.31$_{-0.12}^{+0.15}$ & -3.42$_{-0.024}^{+0.025}$ & 321 \\
 & 23.57$_{-0.12}^{+0.16}$ & -3.86$_{-0.034}^{+0.036}$ & 156 \\
 & 23.84$_{-0.11}^{+0.16}$ & -4.15$_{-0.046}^{+0.052}$ & 81 \\
 & 24.06$_{-0.051}^{+0.22}$ & -4.74$_{-0.084}^{+0.10}$ & 22 \\
 & 24.38$_{-0.10}^{+0.17}$ & -5.25$_{-0.19}^{+0.20}$ & 7 \\
$1.3<z<1.6$ & 23.32$_{-0.16}^{+0.070}$ & -3.36$_{-0.039}^{+0.043}$ & 156 \\
 & 23.53$_{-0.14}^{+0.18}$ & -3.55$_{-0.024}^{+0.025}$ & 323 \\
 & 23.81$_{-0.10}^{+0.21}$ & -4.10$_{-0.037}^{+0.041}$ & 126 \\
 & 24.15$_{-0.12}^{+0.19}$ & -4.53$_{-0.059}^{+0.068}$ & 48 \\
 & 24.39$_{-0.053}^{+0.26}$ & -5.30$_{-0.17}^{+0.18}$ & 8 \\
 & 24.82$_{-0.17}^{+0.14}$ & -5.94$_{-0.37}^{+0.45}$ & 2 \\


==> tab_lumfun_vmax2.tex <==
$1.6<z<2.0$ & 23.55$_{-0.18}^{+0.065}$ & -3.47$_{-0.070}^{+0.084}$ & 156 \\
 & 23.72$_{-0.11}^{+0.18}$ & -3.66$_{-0.024}^{+0.025}$ & 312 \\
 & 23.98$_{-0.080}^{+0.21}$ & -4.15$_{-0.035}^{+0.038}$ & 141 \\
 & 24.28$_{-0.10}^{+0.18}$ & -4.56$_{-0.054}^{+0.062}$ & 57 \\
 & 24.53$_{-0.059}^{+0.23}$ & -5.06$_{-0.092}^{+0.12}$ & 18 \\
 & 24.90$_{-0.14}^{+0.14}$ & -5.86$_{-0.30}^{+0.34}$ & 3 \\
$2.0<z<2.5$ & 23.74$_{-0.15}^{+0.086}$ & -3.61$_{-0.045}^{+0.050}$ & 141 \\
 & 23.94$_{-0.11}^{+0.13}$ & -3.86$_{-0.029}^{+0.031}$ & 219 \\
 & 24.19$_{-0.12}^{+0.13}$ & -4.35$_{-0.042}^{+0.046}$ & 98 \\
 & 24.43$_{-0.11}^{+0.13}$ & -4.71$_{-0.061}^{+0.072}$ & 44 \\
 & 24.66$_{-0.10}^{+0.14}$ & -5.04$_{-0.086}^{+0.11}$ & 21 \\
 & 24.96$_{-0.15}^{+0.092}$ & -5.61$_{-0.20}^{+0.22}$ & 6 \\
$2.5<z<3.3$ & 24.01$_{-0.21}^{+0.079}$ & -3.96$_{-0.051}^{+0.057}$ & 128 \\
 & 24.20$_{-0.11}^{+0.13}$ & -4.21$_{-0.034}^{+0.037}$ & 155 \\
 & 24.42$_{-0.091}^{+0.15}$ & -4.62$_{-0.046}^{+0.051}$ & 81 \\
 & 24.68$_{-0.11}^{+0.13}$ & -4.94$_{-0.065}^{+0.076}$ & 39 \\
 & 24.92$_{-0.11}^{+0.13}$ & -5.43$_{-0.12}^{+0.16}$ & 11 \\
 & 25.18$_{-0.13}^{+0.10}$ & -6.27$_{-0.37}^{+0.45}$ & 2 \\
$3.3<z<4.6$ & 24.30$_{-0.24}^{+0.097}$ & -4.58$_{-0.079}^{+0.096}$ & 55 \\
 & 24.48$_{-0.081}^{+0.12}$ & -5.07$_{-0.077}^{+0.093}$ & 27 \\
 & 24.67$_{-0.074}^{+0.13}$ & -5.24$_{-0.082}^{+0.10}$ & 23 \\
 & 24.86$_{-0.066}^{+0.13}$ & -5.76$_{-0.20}^{+0.22}$ & 6 \\
 & 25.13$_{-0.13}^{+0.067}$ & -5.91$_{-0.22}^{+0.25}$ & 5 \\
$4.6<z<5.7$ & 24.51$_{-0.13}^{+0.085}$ & -4.85$_{-0.15}^{+0.24}$ & 11 \\
 & 24.71$_{-0.12}^{+0.095}$ & -5.50$_{-0.19}^{+0.20}$ & 7 \\
 & 24.88$_{-0.076}^{+0.13}$ & -5.86$_{-0.25}^{+0.28}$ & 4 \\
 & 25.06$_{-0.042}^{+0.17}$ & -6.03$_{-0.30}^{+0.34}$ & 3 \\

